An overview of new measurements of flow, chirality, and vorticity from STAR experiment

In relativistic heavy-ion collisions, the properties of quark-gluon plasma (QGP) and complex dynamics of multi-scale processes in Quantum Chromodynamics (QCD) are studied by analyzing the final state produced particles in a variety of different ways. In these proceedings, we present an overview of new detailed measurements of flow, chirality, and vorticity by the STAR experiment at RHIC. Furthermore, STAR's future opportunities for the precision measurements on small systems, fixed-target (FXT) mode, and Beam Energy Scan (BES-II) program are discussed.

==> Makefile <==
filename=ws-ijmpe

pdf: 
	pdflatex ${filename}
	bibtex ${filename}
	pdflatex ${filename}
	pdflatex ${filename}

open:
	open ${filename}.pdf

clean:
	rm -f ${filename}.ps \
	${filename}.log \
	${filename}.aux \
	${filename}.out \
	${filename}.dvi \
	${filename}.bbl \
	${filename}.blg \
	${filename}.nav \
	${filename}.snm \
	${filename}.toc

